A Hybrid Approach for Learning to Shift and Grasp with Elaborate Motion Primitives

Many possible fields of application of robots in real world settings hinge on the ability of robots to grasp objects. As a result, robot grasping has been an active field of research for many years. With our publication we contribute to the endeavor of enabling robots to grasp, with a particular focus on bin picking applications. Bin picking is especially challenging due to the often cluttered and unstructured arrangement of objects and the often limited graspability of objects by simple top down grasps. To tackle these challenges, we propose a fully self-supervised reinforcement learning approach based on a hybrid discrete-continuous adaptation of soft actor-critic (SAC). We employ parametrized motion primitives for pushing and grasping movements in order to enable a flexibly adaptable behavior to the difficult setups we consider. Furthermore, we use data augmentation to increase sample efficiency. We demonnstrate our proposed method on challenging picking scenarios in which planar grasp learning or action discretization methods would face a lot of difficulties

==> implementation_details.tex <==
\section{Implementation Details}
\label{sec:implementation_details}
\paragraph{Action representation}

Grasping parameters is 3-dim: yaw, pitch, width

Pushing is 5-dim: yaw, pitch, roll, move yaw, move steps

\paragraph{Rewards} Pushing reward is $r(s,a_p)=0$. Grasping reward is $r(s,a_g)=1.0$ if the grasp is successful, and 0 otherwise. 

\paragraph{Episode} An episode terminates if there is a grasp success, otherwise if a maximum number of steps is met. At a new episode, a random heap with domain randomization is generated.

\paragraph{Others} i) object-guided exploration (a simple object detector), ii) double-Q-learning and a recently introduced clipped version \cite{FujimotoHM18}.


==> results_challenging_grasp_only.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental Results for the grasp-only ablation for the Challenging Setting (Mean $\%$)}
    \label{tab:results_challenging}
    \begin{tabular}{c|c|c|c|c}
        Method & Clearance & Completion  & Grasp Succ.  & Action Eff.\\
        \hline
       \cite{berscheid2019robot}  & $23.8$ &    $1.6$   & $7.7$ & $62.3$  
        %\\
         %Ours (cropped image) &0 & $3.3 \pm 0.1$ & 0
        \\
        Ours & $72$ &    $30$   & $33$ & $72$ 
        \\
        \bottomrule
    \end{tabular}
\end{table}

==> results_challenging_unseen.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental Results for grasp-only ablation for the Random Setting (Mean $\%$)}
    \label{tab:results_random_grasp_only}
   \begin{tabular}{c|c|c|c|c}
        Method & Clearance & Completion  & Grasp Succ.  & Action Eff.\\
        \hline
       \cite{berscheid2019robot}  & $33.7$ &    $0.9$   & $11.6$ & $80$
        %\\
        %Ours (cropped image) &$1.0 \pm 1.8$ & $10.5 \pm 1.4$& $44 \pm 0$
        \\
        Ours   & $77$ & $49$       & $39$  & $62$ 
        \\
        \bottomrule
    \end{tabular}
\end{table}


==> results_random_grasp_only.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental Results for grasp-only ablation for the Random Setting (Mean $\%$)}
    \label{tab:results_random_grasp_only}
   \begin{tabular}{c|c|c|c|c}
        Method & Clearance & Completion  & Grasp Succ.  & Action Eff.\\
        \hline
        \cite{berscheid2019robot} & $68.3$ &    $21.7$   & $27.4$ & $64.5$
        %\\
        %Ours (cropped image) &$1.0 \pm 1.8$ & $10.5 \pm 1.4$& $44 \pm 0$
        \\
        Ours   & $85$ & $51$       & $55$  & $85$ 
        \\
        \bottomrule
    \end{tabular}
\end{table}


==> results_random_unseen.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental Results for grasp-only ablation for the Random Setting (Mean $\%$)}
    \label{tab:results_random_grasp_only}
    \begin{tabular}{c|c|c|c|c}
        Method & Clearance & Completion  & Grasp Succ.  & Action Eff.\\
        \hline
        \cite{berscheid2019robot} & $31.9$ &    $1.5$   & $43.5$ & $41.9$
        %\\
        %Ours (cropped image) &$1.0 \pm 1.8$ & $10.5 \pm 1.4$& $44 \pm 0$
        \\
        Ours   & $82.4$ & $53$       & $46$  & $73$ 
        \\
        \bottomrule
    \end{tabular}
\end{table}

